On Structural Explanation of Bias in Graph Neural Networks

Graph Neural Networks (GNNs) have shown satisfying performance in various graph analytical problems. Hence, they have become the \emph{de facto} solution in a variety of decision-making scenarios. However, GNNs could yield biased results against certain demographic subgroups. Some recent works have empirically shown that the biased structure of the input network is a significant source of bias for GNNs. Nevertheless, no studies have systematically scrutinized which part of the input network structure leads to biased predictions for any given node. The low transparency on how the structure of the input network influences the bias in GNN outcome largely limits the safe adoption of GNNs in various decision-critical scenarios. In this paper, we study a novel research problem of structural explanation of bias in GNNs. Specifically, we propose a novel post-hoc explanation framework to identify two edge sets that can maximally account for the exhibited bias and maximally contribute to the fairness level of the GNN prediction for any given node, respectively. Such explanations not only provide a comprehensive understanding of bias/fairness of GNN predictions but also have practical significance in building an effective yet fair GNN model. Extensive experiments on real-world datasets validate the effectiveness of the proposed framework towards delivering effective structural explanations for the bias of GNNs. Open-source code can be found at https://github.com/yushundong/REFEREE.

==> intro_old.tex <==

\section{Introduction}
\label{intro}


Graph Neural Networks (GNNs) have shown satisfying performance on various graph mining tasks, e.g., node classification~\cite{DBLP:conf/iclr/KipfW17}, link prediction~\cite{DBLP:journals/corr/KipfW16a}, etc. Such superiority over traditional graph mining algorithms also makes GNNs popular choices in a variety of decision-making scenarios, such as financial fraud detection~\cite{wang2019semi}, recommendation~\cite{fan2019graph}, and recidivism predictions~\cite{agarwal2021towards}. The success of GNNs is generally attributed to its painstakingly designed message-passing mechanism~\cite{wu2020comprehensive,zhou2020graph}. Such mechanism broadly enables GNNs to capture the localized correlation between any node and its neighbors, which helps to extract information from both attribute and structure into the learned node embeddings~\cite{velivckovic2017graph,hamilton2017inductive}.

However, despite the remarkable success GNNs have achieved, they are never flawless: most existing GNNs do not have fairness consideration~\cite{dong2021individual,dong2021edits,dai2021say}. As a consequence, the wide-spreading utilization of GNNs in high-stake application scenarios (e.g., medical diagnosis~\cite{saha2021graphcovidnet}) raises the societal concern about the algorithmic fairness issue~\cite{kang2021fair}. 
%
As a matter of fact, how to promote fairness for machine learning algorithms has long been a critical challenge in myriads of decision-making scenarios~\cite{mehrabi2021survey,du2020fairness,madras2018learning,chang2020adversarial}. For example, sensitive attributes such as gender and skin color could severely affect the algorithm performance on facial recognition for the demographic groups with certain sensitive features~\cite{buolamwini2018gender}.
%
Similarly, the fairness issue of GNNs has also attracted much research attention.
%
For example, some existing works promote GNNs performance on fairness via adversarial learning to decouple the learned embeddings from sensitive features~\cite{dai2021say}.
%
However, what exactly leads to a biased GNN?
%
Up to now, one of the convincing assumptions is that the bias exhibited in GNNs is resulted from the biased input network data itself~\cite{DBLP:conf/iclr/LiWZHL21,dong2021edits,jalali2020information,spinelli2021biased,kose2021fairness}. 
%
For example, some fairly recent works have empirically proved that the bias of the input network data is a significant source of bias for GNNs~\cite{DBLP:conf/iclr/LiWZHL21}, as such data bias could be retained or amplified by the core operation of GNNs -- the message-passing mechanism~\cite{dong2021edits}.
%
In this regard, it would be difficult to obtain a fair GNN with biased training data~\cite{du2020fairness}.

To relieve the bias in the input network data, which potentially leads to less biased GNNs, various efforts have been made recently.
%
For example, Jalali et al.~\cite{jalali2020information} define information unfairness score based on the information flow between nodes from different sensitive group (i.e., groups divided w.r.t. sensitive attributes), and propose an algorithm to maximally reduce such score through removing edges; Dong et al.~\cite{dong2021edits} propose to learn a less biased weighted graph topology based on the embedding distribution difference between two sensitive groups; Li et al.~\cite{DBLP:conf/iclr/LiWZHL21} optimize adjacency matrix to minimize the expected linkage probability difference between inter- and intra-group node pairs.
%
As is clearly observed from these recent efforts, how to relieve biased structure of the input network data of GNNs has become a critical concern.
%
Nevertheless, despite the existing efforts on modifying the input network structure towards a less biased GNN, to the best of our knowledge, no existing work explicitly scrutinizes the patterns in the network structure that influence the bias level of the GNN prediction for a specific node.
%
Generally, given a specific node, the GNN prediction is only determined by the corresponding localized subgraph centered on the given node (i.e., the computation graph of this node).
%
Consequently, to explain what leads to a biased prediction for a specific node, identifying the biased structure patterns in the corresponding computation graph is critical.
%
Towards this goal, a few recent works are able to provide us some preliminary insights. For example, some fairly recent works argue that in any computation graph, those intra-group edges according to the sensitive feature lead to bias in the process of embedding learning~\cite{spinelli2021biased};
% 有些人说inter group的link少就会导致bias
however, inter-group edges are also found to introduce or exaggerate bias in GNNs through the message-passing mechanism~\cite{dong2021edits}. % 但是inter group的link多却不合适也会导致，比如一个toy example
%
Beyond that, in real-world scenarios, the network subgraph structure patterns that cause bias could be much more complicated than we can imagine, and a mixture of different subgraph structure patterns could either introduce bias or promote fairness in the training of a certain GNN.
%
As a consequence, existing works only contribute rather limited understanding to the patterns in the computation graph structure that lead to biases in GNNs for a specific node.
%
However, considering the significance of fair GNNs in various applications, we argue that it is highly urgent to provide localized structural explanations on the bias in networks towards a better understanding of the bias exhibited in GNNs.


Towards the goal of obtaining localized structural explanations to identify what causes bias in GNNs given a specific node, a natural idea is to resort to the existing GNN-based explanation models~\cite{luo2020parameterized,ying2019gnnexplainer,yuan2021explainability,schlichtkrull2020interpreting,huang2020graphlime,vu2020pgm,dai2021towards}.
%
% Generally, for any GNN explanation model, the goal towards better utility is to achieve better sparsity and fidelity~\cite{yuan2020explainability}. Sparsity requires that the explanation should be the smallest edge set that maximally influence the prediction of the center node, while fidelity emphasizes that the prediction of the center node should be minimally influenced with the learned edge mask.
%
Nevertheless, existing GNN-based explanation models only capture the high-impact localized subgraph structure w.r.t. a given prediction. To the best of our knowledge, no existing GNN-based explanation model is able to identify how each edge in a localized subgraph influences the bias level for the prediction of the corresponding node.
%
In other words, the explanation given by existing GNN-based explanation models is too coarse to identify the contribution difference across edges to the bias exhibited in GNNs, e.g., answering whether an edge leads to a more biased or fair prediction for a node.  %不能更细粒度地给出解释 too to
%
As a result, it is impractical to directly adopt existing GNN-based explanation models to identify the contribution of each edge to the bias level for any specific node in GNNs.


To provide a better understanding of how different edges in the input network of GNNs contribute to the bias, in this paper, we investigate a novel problem of \textit{structural explanation of biases in Graph Neural Networks}. Nevertheless, developing a framework to identify how each edge in the localized subgraph structure contribute to the bias for the prediction of a given node is non-trivial. Essentially, we mainly face the following three challenges:
%
(1) \emph{\textbf{Fairness Notion Gap}}. Studying how each edge in the localized subgraph structure contribute to the bias of the given prediction naturally requires to dive into the node level. However, existing group fairness notions are defined based on the whole population. As a consequence, how to build the gap between such macro-level and the micro-level group fairness notions is the first and foremost challenge;
%
(2) \emph{\textbf{Low Granularity}}. As mentioned above, existing GNN-based explanation approaches only provide explanation at a lower granularity, i.e., they cannot explicitly identify how each edge influences the given node prediction from the perspective of fairness. Hence how to design a framework to provide structural explanation at a higher granularity is the second challenge; and
%
(3) \emph{\textbf{Lack of Ground Truth}}. Considering the complexity of the real-world networks, the ground truth of how each localized edge influences the fairness level of the given node prediction is unavailable. In this regard, it would also be challenging to properly formulate constraints for the developed framework towards accurate explanations.

As an attempt to solve the challenges above, we propose VISION (contrasti\underline{V}e learn\underline{I}ng towards \underline{S}tructural explanat\underline{I}ons f\underline{O}r the fairness of G\underline{N}Ns) in this paper.
%
To dive into the node level to handle the first challenge, we propose a novel bias metric to justify how bias the prediction is for a specific node . %It should be noted that the proposed metric is consistent with traditional group fairness notions. 
%
We then formulate a novel problem of \textit{structural explanation of biases in Graph Neural Networks}.
%
To tackle the second challenge, we propose a model-agnostic framework for post-hoc GNN explanation named VISION towards more granular explanation. VISION is agnostic for both GNNs and the corresponding post-hoc explanation models. Such dual-agnostic characteristic equips VISION with better generalization ability and flexibility.
%
For the last challenge, we design a training scheme based on contrastive learning to avoid the use of ground truth labels. Finally, we evaluate the effectiveness of our proposed framework on real-world network datasets.
%
The main contributions of this paper is summarized as follows.
\begin{itemize}
    \item \textbf{\emph{Problem Formulation.}} We study a novel problem of structural explanation of biases in GNNs. A novel metric is proposed to determine how much a specific node contribute to the overall bias for the prediction of GNNs.
    \item \textbf{\emph{Algorithmic Design.}} We address the limitation of GNN explanation models, and propose a novel model-agnostic explanation framework VISION to identify edges that promote and reduce bias for a given node in the GNN input network.
    \item \textbf{\emph{Experimental Evaluations.}} We perform comprehensive experimental evaluations on real-world attributed networks. The effectiveness and superiority of VISION is validated through experiments.
\end{itemize}

